PyRobot: An Open-source Robotics Framework for Research and Benchmarking

This paper introduces PyRobot, an open-source robotics framework for research and benchmarking. PyRobot is a light-weight, high-level interface on top of ROS that provides a consistent set of hardware independent mid-level APIs to control different robots. PyRobot abstracts away details about low-level controllers and inter-process communication, and allows non-robotics researchers (ML, CV researchers) to focus on building high-level AI applications. PyRobot aims to provide a research ecosystem with convenient access to robotics datasets, algorithm implementations and models that can be used to quickly create a state-of-the-art baseline. We believe PyRobot, when paired up with low-cost robot platforms such as LoCoBot, will reduce the entry barrier into robotics, and democratize robotics. PyRobot is open-source, and can be accessed via https://pyrobot.org.

==> class-projects.tex <==
\begin{figure*}
    \centering
    \includegraphics[height=0.21\linewidth]{figures/cmu-class/lego.png}
    \includegraphics[height=0.21\linewidth]{figures/cmu-class/chess.png}
    \includegraphics[height=0.21\linewidth]{figures/cmu-class/trash.png}
    \includegraphics[height=0.21\linewidth]{figures/cmu-class/butler.png}
    \caption{Example projects undertaken by students using \locobot. Photo Credit: Oliver Kroemer, Timothy Lee, Mohit Sharma, Ganesh Iyer, Lukas Merkle, Rohan Tiwari, Karun Warrior, Stanley Winata, Angela Chao, John Macdonald, Rupika Nilakant, Atulya Ravishankar, Akshit Gandhi, Shubham Garg, Parv Parkhiya, Zhihao Zhu, Hillel Hochsztein, Aubrey Kalashian, Joshua Ra'anan, Apoorv Singh. \todo{We should decide if we want to keep this figure and all the names or not.}}
    \label{fg:education}
\end{figure*}

==> grasping-code.tex <==
\begin{listing}
\caption{Grasping example using \pyrobot API.}
\label{code:grasping}
\begin{minted}{python}
from pyrobot import Robot
import numpy as np

# Construct Robot.
bot = Robot('locobot')

# Set some variables
reset_pos = [-1.5, 0.5, 0.3, -0.7, 0.]
pregrasp_height = 0.2
grasp_height = 0.13

# Construct grasp model.
model = GraspModel()

# Set goal for policy.
while True:
    # Move arm and camera to reset position
    bot.arm.set_joint_positions(reset_pos)
    bot.camera.set_pan_tilt(0.0, 0.8)
    
    # Get image.
    rgb = bot.camera.get_rgb()
    
    # Compute action.
    grasp_img = model.compute_grasp(rgb)
    
    # Convert grasp from Image space to 
    # Robot workspace
    grasp_pose = cvt_space(grasp_img)
    
    # Execute grasp.
    ## Go to pre-grasp pose
    pregrasp_position = [grasp_pose[0],
                         grasp_pose[1],
                         pregrasp_height]
    grasp_angle = grasp_pose[2]
    bot.arm.set_ee_pose_pitch_roll(
        position=pregrasp_position,
        pitch=np.pi / 2,
        roll=grasp_angle,
        plan=False,
        numerical=False)
    ## Go to grasp pose
    grasp_position = [grasp_pose[0],
                      grasp_pose[1],
                      grasp_height]
    bot.arm.set_ee_pose_pitch_roll(
        position=grasp_position,
        pitch=np.pi / 2,
        roll=grasp_angle,
        plan=False,
        numerical=False)
    ## Grasp the object
    bot.gripper.close()
\end{minted}
\end{listing}

==> pushing-code.tex <==
\begin{listing}
\caption{Pushing example using \pyrobot API.}
\label{code:pushing}
\begin{minted}{python}
from pyrobot import Robot
import numpy as np

# Construct Robot.
bot = Robot('locobot')

# z coordinate of the floor
z_th = 0.0

# Setup gripper, camera, arm
bot.gripper.close()
bot.camera.set_pan_tilt(0, 0.7, wait=True)
bot.arm.go_home()


# Move hand out of camera view.
ov_pos = [1.96, 0.52, -0.51, 1.67, 0.01]
bot.arm.set_joint_positions(ov_pos, plan=False)

# Get the point cloud(in base frame).
pts, colors = bot.camera.get_current_pcd(
                  in_cam=False)
# Filter point cloud 
# (remove floor and far points)
pts, colors = filter_points(pts, colors, 
                            z_lowest=z_th)
# Project the remaining point
# cloud onto xy-plane                             
xy_pts = pts[:, :2]
# Use DBSCAN to cluster the points
labels = segment_objects(xy_pts)
# sample an object and a
# start point for pushing
tgt_pts = sample_pt(pts, labels)
pre_push_pt, push_pt, obj_center = tgt_pts

# Move the gripper to pre-pushing pose
bot.arm.set_ee_pose_pitch_roll(
    position=pre_push_pt,
    pitch=np.pi / 2,
    roll=0,
    plan=False,
    numerical=False)
                               
# Move the gripper vertically down
down_disp = push_pt - pre_push_pt
bot.arm.move_ee_xyz(down_disp, 
                    plan=False, 
                    numerical=False)

# Move the gripper horizontally
# to push the object
hor_disp = 2 * (obj_center - push_pt)
bot.arm.move_ee_xyz(hor_disp, 
                    plan=False, 
                         numerical=False)
\end{minted}
\end{listing}
